Agreement testing theorems on layered set systems

We introduce a framework of layered subsets, and give a sufficient condition for when a set system supports an agreement test. Agreement testing is a certain type of property testing that generalizes PCP tests such as the plane vs. plane test. Previous work has shown that high dimensional expansion is useful for agreement tests. We extend these results to more general families of subsets, beyond simplicial complexes. These include - Agreement tests for set systems whose sets are faces of high dimensional expanders. Our new tests apply to all dimensions of complexes both in case of two-sided expansion and in the case of one-sided partite expansion. This improves and extends an earlier work of Dinur and Kaufman (FOCS 2017) and applies to matroids, and potentially many additional complexes. - Agreement tests for set systems whose sets are neighborhoods of vertices in a high dimensional expander. This family resembles the expander neighborhood family used in the gap-amplification proof of the PCP theorem. This set system is quite natural yet does not sit in a simplicial complex, and demonstrates some versatility in our proof technique. - Agreement tests on families of subspaces (also known as the Grassmann poset). This extends the classical low degree agreement tests beyond the setting of low degree polynomials. Our analysis relies on a new random walk on simplicial complexes which we call the ``complement random walk'' and which may be of independent interest. This random walk generalizes the non-lazy random walk on a graph to higher dimensions, and has significantly better expansion than previously-studied random walks on simplicial complexes.

==> sections/high_dim_sets.tex <==
\begin{proof}[Proof of \pref{thm:main-agreement-theorem-two-sided}]
First, note that when $d$ is small, the theorem is true by a simple union bound. Thus we may assume $d>>1$.

To show the theorem is true, we need to take some ensemble of functions $\FF$ and show that if $\disagr(\FF) = \varepsilon$ then there exists a global function $G: X(0) \to \Sigma$ such that
\[ \Prob[s \sim D_{d,\ell}]{f_s \ane{\frac{r}{\ell}} \rest{G}{s}} = c \left ( 1 + \frac{1}{r} \right ) \varepsilon, \]
for some constant $c$.


Denote by 
\[ S' = \sett{(s_1,...,s_j)\in X(d)}{\exists t\in X(\ell)\; t \subset \bigcap_{i=1}^j s_i}.\]
\[T' = X(t); A' = X(t-1); V' = X(0). \]

Our STAV-structure is
%Complete%
Our distribution is
\begin{enumerate}
    \item Choose $t \in X(\ell)$
    \item Choosing $(s_1,...,s_{j+1}) \in S$ according to the distribution of the simplicial complex. All the $s_i$ are chosen independently.
    \item Choosing $(v,a)$ by choosing $v \in t$ uniformly at random and setting $a = t \setminus \set{v}$.
\end{enumerate}
The $STS$-test of this structure is by
\begin{enumerate}
    \item Choose $t \in X(\ell)$
    \item Choosing $(s_1,...,s_{j+1}),(s_{j+2},...,s_{2j+2}) \in S$ according to the distribution of the simplicial complex. All the $s_i$ are chosen independently.
\end{enumerate}

The $\VASA$-distribution is the following:
\begin{enumerate}
    \item Choose $(s_1,...,s_{j+1}) \in X(d)$.
    \item Choose $a_1,a_2,v$ so that $a_1 \dunion a_2 \dunion \set{v} \subset \bigcap_{i=1}^j s_i$.
\end{enumerate}
This distribution is obviously symmetric in $a_1$ and $a_2$. Furthermore, the choice of $(v,a_i,\vec{s})$ is identical to the marginal in the STAV-structure.
We cannot use the ensemble function $\FF$ as is. Instead we define 
\[ \tilde{\FF} = \sett{f_\vec{s}:\binom{\cap \vec{s}}{j+1} \to \Sigma^{j+1}}.\]
Where $f_{\vec{s}}(v) = (f_{s_1}(v),...,f_{s_{j+1}}(v))$.
Note that if $f_{\vec{s}}(v) = f_{\vec{s'}}(v)$ if and only if for every coordinate $i$, $f_{s_i}(v) = f_{s'_i}(v)$. Hence $?$

If we will find a global function


First, we claim that for any simplicial complex, the STAV-structure above has $\surp(X) = \bigO{k^{-j}}$.

\begin{proof}[Proof of \pref{claim:agreement-on-last-vertex}]
Let $\FF$ be any ensemble of local functions. We need to show that 
\[ \cProb{(s_1,s_2,t,a)}{\rest{f_{s}}{a} = \rest{f_{s}}{a}}{\rest{f_{s}}{t} = \rest{f_{s}}{t}}.\]
To do so, we want to invoke \pref{lem:delta-surprise}. For every $t \in T$, the $T$-lower graph is the containment graph where on one side we have
\[ L = \binom{t}{\ell-1},\]
and on the other we have
\[ R = \set{v \in t}.\]
%The next paragraph is not implied by \cite{KaufmanO2018} that only promines 1/\sqrt{\ell}%
It is a well known fact that this graph is a $\frac{1}{\ell}$-bipartite expander. Trivially, if $\rest{f_{s_1}}{t} \ne \rest{f_{s_2}}{t}$, they differ on at least $\frac{1}{\ell+1}$-fraction of the vertices (namely, one vertex). By \pref{lem:delta-surprise}, we get a surprise of $\frac{\ell^{-2}}{(\ell+1)^{-1}} = \bigO{\frac{1}{\ell}}$.
\end{proof}

If we show STAV-structure defined above theorem is $\bigO{\gamma}$-good as in \pref{def:good-stav-structure}, for $\gamma = \frac{1}{\ell}$, we could invoke \pref{thm:main-STAV-agreement-theorem} and conclude. Hence we need, that it fulfils the assumptions in \pref{def:good-stav-structure}:
\begin{enumerate}

    \item We begin with the proof of \pref{ass:a-not-large}. We require that the probability of choosing some $v \in s$ so that $v \in \adj{a}$ is greater or equal to $\frac{1}{2}$ for any $a \subset s$. as $\ell < \frac{1}{2}d$, and $s \cap \adj{a} = s \setminus a$ for any $a \subset s$,
    \[ \cProb{}{v \in \adj{a}}{v \in s} = \frac{|s \setminus a|}{|s|} \geq \frac{1}{2}.\]
    %%%   {This is at the beginning on purpose. I think it is better to put it here than to put it in the end, where it hides after spectral claims.}   %%%

    \item \pref{ass:global-A-V-graph}: The graph described in this assumption is the $0,\ell-1$ complement walk graph in $X$. By our assumption $X$ is a $\frac{1}{d^2 \ell}$-two-sided HDX. Thus from \pref{claim:two-sided-complement-walk-is-a-good-expander}, this graph is a $\bigO{\frac{1}{\ell}}$-bipartite expander.

    \item \pref{ass:edge-expander}: Fix $a \in A$. The conditioned $STS$-graph, $STS_{a}$ is the graph whose vertices are all $\ul{a}{s}$. Traversing from $s_1$ to $s_2$ is going by $t = a \dunion \set{v}$. We are to show that this graph is a $\bigO{\frac{1}{\ell}}$-two-sided spectral expander. Indeed this graph is (isomorphic to) the graph obtained whose vertices are $X_a(d - \ell)$, and $s_1 \setminus a, s_2 \setminus a$ are connected by an edge if their intersection contains a vertex in $X_a(0)$. $d-\ell = \Omega(\ell)$ thus by \pref{thm:containment-graph-is-a-good-expander}, and the fact that $X$ is an $\frac{1}{\ell d^2}$-HDX, this graph is a $\eta$-two-sided spectral expander, for
    \[ \eta = \frac{1}{d- \ell} + \bigO{\frac{d}{d^2 \ell}} = \bigO{\frac{1}{\ell}} = \bigO{\gamma}. \]
     In particular, it is an $\frac{1}{3}$-edge-expander (for a large enough $d$).

    \item \pref{ass:v-a-graph}:
    We are to bound the spectral gap in the conditioned $STS$-graph, namely $STS_{a,v}$, whose vertices are $s \supset (a,v)$, and edges are $(s_1,t,s_2)$ where $t \supset (a,v)$.

    In the context of the STAV-structure above, conditioning on $a \in A, v \in X(0)$ is the same as conditioning on $t = a \dunion \set{v} \in T$. In this case, the choices of $s_1,s_2$ are independent - i.e. the graph we get is a clicque with self loops. This graph is a $0$-two-sided spectral expander.

    \item \pref{ass:vasa-graphs-v}: Fix some $v \in V$. The $\vASA{v}$-graph is the graph whose vertices are all $a,a'$ so that $(v,a,s,a')$ are in the support of the $\VASA$-distribution. In this case these are exactly $X_v(\ell-1)$. We go from $a$ to $a'$ by choosing $(v,a,s,a')$ in the $\VASA$-distribution. Thus in this case we go from $a$ to $a'$ if they are disjoint and share a face $s \setminus \set{v} \in X_v(d-1)$.

    The graph we just described is the $(\ell-1),(\ell-1)$-complement walk graph in $X_v$, the link of $v$. $X$ is a $\bigO{\frac{1}{\ell d^2}}$-two-sided HDX, thus by \pref{claim:two-sided-complement-walk-is-a-good-expander}, this graph is a $\ell^2\bigO{\frac{1}{\ell d^2}} = \bigO{\frac{1}{\ell}}$-bipartite expander.

    \item \pref{ass:vasa-graphs-a}: This is the only part of the proof that is not immediate. Fix some $a \in A$. The graph in this assumption is the $\VAS{a}$-graph, the bipartite graph where
    \[ L = \adj{a_0}, \; R = \sett{(a,s)}{\exists v \in L \; (v,a_0,s,a) \in Supp(D) },\]
    \[ E = \set{(v,(a,s)) : (v,a_0,s,a) \in Supp(D) }. \]
    The probability of choosing an edge $(v,(a',s))$ is given by $\cProb{D}{(v,a_0,s,a')}{a_0 = a}$.

    We describe the graph in this case explicitly in this following proposition, that says this graph is a $\sqrt{\gamma}$-bipartite expander.

    \begin{proposition}
        \label{prop:two-sided-graph}
    Fix some $a \in A$, and consider the following graph
    \begin{itemize}
        \item $L = \set{(a', s) : a' \dunion a \subset s}.$
        \item $R = \adj{a} = X_a(0).$
        \item $E = \set{(v,(a',s)) : \set{v} \dunion a' \dunion a \subset s},$ and the probability to choose each edge is given by the distribution that chooses $(s, a', v)$ in the link of $a$.
    \end{itemize}

    The graph described above is an $\bigO{\frac{1}{\sqrt{\ell}}}$-bipartite expander.
\end{proposition}

\begin{figure}
    \centering
    \includegraphics[]{graphics/two-sided-vas_a.PNG}
    \caption{A triangle in $Y$. }
    \label{fig:my_label}
\end{figure}

To prove this proposition, we state \pref{lem:structure-trickling-lemma}. The proof of this lemma uses Garland's method, so we postpone its proof to \pref{sec:complement-walk}.

\begin{lemma}
    \torestate{
    \label{lem:structure-trickling-lemma}
    Let Y be a $2$-dimensional $3$-partite complex, and denote its parts by $X(0) = X[1] \dunion X[2] \dunion X[3]$. Suppose that for every $v \in X[1]$, $X_v$ is a $\eta$-bipartite expander. Denote by $A^{1,2}$, $A^{1,3}$  and $A^{2,3}$ the bipartite walks between $(V_1,V_2)$ $(V_2,V_3)$ and $(V_2,V_3)$ respectively. Then
    \[ \lambda (A^{2,3}) \leq \eta + \lambda(A^{1,2}) \lambda(A^{1,3}) . \]
    }
\end{lemma}

    \begin{proof}[Proof of \pref{prop:two-sided-graph}]
    Consider the following $2$-dimensional $3$-partite simplicial complex:
    \begin{itemize}
        \item The parts of the complex are $Y[1] = X_a(t-1), Y[2] = X_a(0), Y[3] = \sett{(a', s) \in X(t-1) \times X(d)}{a \dunion a' \subset s}$.
        \item We connect $(a',v,(a'',s)) \in Y(2)$ if $a' = a''$ and $\set{v} \dunion a' \dunion a \subset s$. The probability of choosing some triangle $(a',v,(a'',s))$ is the probability of choosing $s$ given $a$, and then choosing $a', v$ (given that they are disjoint from $a$): \[\cProb{X}{s}{a}\cProb{X}{a'}{s \setminus a}\cProb{X}{v}{s \setminus (a \dunion a')}. \]
    \end{itemize}
    We notice the following:
    \begin{enumerate}
        \item $A^{2,3}$ is the bipartite operator of the bipartite walk between $L,R$ in the we defined in the proposition.
        \item $A^{1,2}$ is the bipartite operator of the complement walk in the link of $a$, and from \pref{claim:two-sided-complement-walk-is-a-good-expander} $\lambda(A^{1,2}) \leq d^2 \lambda(X_a) = \bigO{\frac{1}{\ell}}$.
        \item for every $a' \in Y\sqbrack{1}$, the bipartite operator of the link of $a'$ is the containment walk between $X_{a \dunion a'}(0)$ and $X_{a \dunion a'}(d-2\ell)$. Recall that $\frac{1}{2}d - \ell = \Omega(d)$, thus $d-2\ell = \Omega(d)$. Hence this walk is also an $\bigO{\frac{1}{\sqrt{\ell}}}$ expander.
    \end{enumerate}
    Hence we can apply \pref{lem:structure-trickling-lemma} and conclude that
    \[ \lambda(A^{2,3}) \leq \bigO{\frac{1}{\sqrt{\ell}}} + \bigO{\frac{1}{\ell}} = \bigO{\frac{1}{\sqrt{\ell}}}.\]
    \end{proof}
\end{enumerate}
\end{proof}
